Empirical Characterization of Mobility of Multi-Device Internet Users

Understanding the mobility of humans and their devices is a fundamental problem in mobile computing. While there has been much work on empirical analysis of human mobility using mobile device data, prior work has largely assumed devices to be independent and has not considered the implications of modern Internet users owning multiple mobile devices that exhibit correlated mobility patterns. Also, prior work has analyzed mobility at the spatial scale of the underlying mobile dataset and has not analyzed mobility characteristics at different spatial scales and its implications on system design. In this paper, we empirically analyze the mobility of modern Internet users owning multiple devices at multiple spatial scales using a large campus WiFi dataset. First, our results show that mobility of multiple devices belonging to a user needs to be analyzed and modeled as a group, rather than independently, and that there are substantial differences in the correlations exhibited by device trajectories across users that also need to be considered. Second, our analysis shows that the mobility of users shows different characteristics at different spatial scales such as within and across buildings. Third, we demonstrate the implications of these results by presenting generative models that highlight the importance of considering the spatial scale of mobility as well as multi-device mobility. More broadly, our empirical results point to the need for new modeling research to fully capture the nuances of mobility of modern multi-device users.

==> analysis.tex <==
\section{Empirical Analysis of user devices}
\label{sec:analysis}

In today's world, most of us carry more than one mobility device. In our study, we found that each mobile device associated with a user has it's own mobility trace and displays different mobility characteristics. In this section we share the results of empirical analysis of the multiple user devices associated with a user. We divide all the mobile devices associated with a user in 3 different categories. Of all the devices associated with a user, the device that shows the most mobility is termed as a primary device. The next most mobile device is termed as secondary device followed by tertiary and other devices. We also divide the users in 2 distinct groups of students and faculty/staff. 

In a campus environment a user visits a location spends some time at that location performing some activity. Most of the users move between locations spending different amount of time at different locations. We term the locations visited by the users as Locations of Interest [LoI]. We found that a lot of users displayed the behaviour of revisiting few LoI's over the course of the day.

In the below subsections we present the mobility characteristics of primary, secondary, tertiary and other devices.

\subsection{Primary Device Analysis}

%\begin{figure*}
%\begin{tabular}{cc}
%	\includegraphics[width=3.1in]{./Figures/faculty_mean_unique_bldgs_visited_by_day.pdf}&
%	\includegraphics[width=3.1in]{./Figures/students_mean_unique_bldgs_visited_by_day.pdf}\\
%(a) Faculty/Staff & (b) Students
%\end{tabular}
%\vspace{-0.2in}
%\caption{Mean number of unique LoI's visited by day of week}
%\vspace{-0.05in}
%\label{fig:LoI_mean_unique_visits}
%\end{figure*}

\begin{figure}[H]
\includegraphics[width=3.1in]{./Figures/plt_LoI_histogram_entire_dataset_concatenated_dates_LOI_file.pdf}\\
\vspace{-0.2in}
\caption{Number of Unique LoI's visited by role for entire semester}
\vspace{-0.05in}
\label{fig:LoI_unique_visits_dataset_pri}
\end{figure}

Figure ~\ref{fig:LoI_unique_visits_dataset_pri} shows the number of unique locations visited by the primary device of users over the course of a semester. We find that about 87\% of the staff visit 3 or less unique locations per day whereas, about 75\% of students visit upto 4 unique locations per day. This shows that students visit more number of unique buildings over the course of a day and have higher mobility as compared to staff. Since, a large percentage of our population comprises of students who usually take 3 or more courses over a semester, the primary device owned by students displays high mobility. On the other hand, faculty and staff usually limit their visits to their office, office hours room or classroom for the course taught, this results in less number of unique buildings visited than that of students.

\begin{figure}[H]
\begin{tabular}{cc}
	\includegraphics[width=3.1in]{./Figures/faculty_mean_LoI_visited_by_day.pdf}&
	\includegraphics[width=3.1in]{./Figures/students_mean_LoI_visited_by_day.pdf}\\
(a) Faculty/Staff & (b) Students
\end{tabular}
\vspace{-0.2in}
\caption{Mean number of LoI's visited by day of week}
\vspace{-0.05in}
\label{fig:LoI_mean_visits_pri}
\end{figure}

In Figure ~\ref{fig:LoI_mean_visits_pri} we show the mean number of locations visited by users on different days of the week. We find that while faculty/staff show an almost constant mean number of locations visited of about 2.5 locations across the days of the week, students show a wider range of mean locations visited from about 4 to ~6 based on the day of the week. This shows, that there is high variance in daily schedules of the student population. Also, for both user groups we find that weekends show less mobility compared to weekdays. For the student population, Wednesday shows most mobility while Friday shows least mobility of all weekdays.

\begin{figure}[H]
\includegraphics[width=3.65in]{./Figures/Percentage_time_dist_stacked.pdf}\\
\vspace{-0.2in}
\caption{Percentage time spent across locations over a course of day}
\vspace{-0.05in}
\label{fig:time_dist_pri}
\end{figure}

Figure ~\ref{fig:time_dist_pri} shows the percentage time spent across locations over a course of a day. Users who visit only one unique location spent all their time at that location. However, as the number of unique locations visited increases we find that the users tend to spend a majority of their day at a particular location and distribute the rest of the time across other locations. We analyse the percentage time spent across locations for different users who visit 1-8 unique locations over the course of the day and we found that irrespective of the number of locations visited users tend to spent atleast 50\% of their time at one particlar location and divide the rest of their time across other locations visited. For the student population who live on-campus dorm was the location where on-campus students spend a big chunk of their time. Faculty and staff tend to spend a large amount of time in their location of work or office. 



==> bldg_analysis.tex <==
\subsection{Buildings and Campus}
\label{sec:bldg_analysis}

In this section, we analyze the distribution of building types on campus and activeness of devices by building type. The main questions we answer in this section are:
\begin{itemize}
    \item How many and what type of buildings do we have on campus?
    \item How do we identify on-campus and off-campus users? What is the percentage of on-campus and off-campus users? 
    \item How frequently do users come to campus?
    \item Does device activeness depend on the building type the user is in?
    \item Can we track inter-building and inside-building device trajectories?
\end{itemize}

%\begin{figure*}
%\begin{minipage}[c]{0.48\linewidth}
%\includegraphics[width=\linewidth]{./Figures/bldg_dist_pie_chart.pdf}
%\caption{Distribution of buildings on campus by type: This figure shows the percentage distribution of buildings by the type of activities conducted inside the building. There are 11 building types with Dorm and Educational buildings constituing the largest percentageof buildings on campus.}
%\vspace{-0.05in}
%\label{fig:bldg_types}
%\end{minipage}
%\hfill
%\begin{minipage}[c]{0.48\linewidth}
%\includegraphics[width=\linewidth]{./Figures/user_visit_by_day.pdf}
%\vspace{-0.2in}
%\caption{Distribution of Number of users on campus by role: Tuesday, Wednesday, Thursdays have highest campus visits with least variance for all users. Mondays show high variability and less users. Fridays see least mean among all weekdays since few classes are scheduled on Friday. On-campus student population constitutes to the weekend student users on campus. Also, Sunday sees an increase in student users because off-campus students visit educational buildings, labs and dining services on sundays to either work on their research and coursework or for dining needs.}
%\vspace{-0.05in}
%\label{fig:campus_visits}
%\end{minipage}%
%\end{figure*}

\begin{figure*}
\begin{tabular}{cc}
    \includegraphics[width=3.1in]{./Figures/device_active_bldg_weekday.pdf}&
    \includegraphics[width=3.1in]{./Figures/device_active_bldg_weekend.pdf}\\
(a) Weekdays & (b) Weekends
\end{tabular}
\vspace{-0.2in}
\caption{Device Activness by buildings on weekdays and weekends. Percentage Stacked Bar plot shows the building types across which the devices are most active on Weekday and Weekends. Secondary and Tertiary devices are accessed less in dining, rec-center, parking , etc. Building type impacts the usage of device type.}
\vspace{-0.05in}
\label{fig:device_activeness_by_bldg}
\end{figure*}

We analyze 156 buildings on campus divided into 11 main categories based on the activities performed inside the building. The 11 categories are the dormitory, education, recreation, dining, student organization, administration, parking, health services, events, library and police department. The percentage distribution of buildings present on campus based on the activities is shown in Figure ~\ref{fig:bldg_types}. We see that dormitory and educational buildings comprise of 76.6\% of all campus buildings. The student population that lives in the residential buildings on campus or dormitories is labeled as on-campus students, whereas student population who do not reside in the dorms is labeled as off-campus students. From the dataset, we identify that ~60\% of students are on-campus students. 
\par
Figure ~\ref{fig:campus_visits} shows the distribution and variance of campus visits by students and faculty/staff across the days of a week. We find that while Tuesday, Wednesday, and Thursday shows a high number of all users and has the least variance, Mondays show the highest variance for faculty, staff and student users. For faculty, staff and students Tuesday sees most attendance on campus with least variability, while Friday sees the least attendance for a weekday, the reason being fewer classes are scheduled on Fridays compared to the rest days of the week. On-campus students mostly contribute to the student users footprints on the weekend while we see a sharp drop in the faculty and staff visits on weekend. Saturdays see the least number of student users on campus and show a high variability. Also, a lot of student parties and activities happen outside the campus on Saturday resulting in less user presence on campus. We find that few off-campus students visit educational buildings, labs and dining halls on Sundays to work on research, courses or for dining, increasing the campus user count on Sunday.
\par
In the earlier subsection, we saw that different mobile devices owned by the same user show different mobility trends. We further wanted to analyze if each device type has specific building types where they are accessed more. Figure ~\ref{fig:device_activeness_by_bldg} shows the percentage time the devices were active across buildings. We find that on Weekdays primary devices were mainly accessed in dorms for 52\% of their registered time on the network while secondary devices were accessed ~63\% of the registered time in dorms and tertiary devices were accessed ~68\% of the registered time in dorms. We also see that secondary and tertiary devices are accessed relatively infrequently in dining halls and recreation centers. Another observation we made from the data is that while primary devices were access across all durations of stay, secondary and tertiary devices were used mainly in longer stationary segments of the user trajectory. So, locations, where students tend to spend a longer percentage of their time such as a dorm or educational building, tends to show higher usage of the secondary or tertiary devices than the locations where they spent a smaller percentage of their time or have a shorter visit such as parking services, health services, and administration office. Also, activity performed impacts the device activeness eg. in a dining hall and in a recreation center the usage of secondary and tertiary devices is very low compared to the usage of the primary device. Figure ~\ref{fig:device_activeness_by_bldg} (b) shows a similar weekend trend with a heavier access in dorms due to the absence of classes on weekdays resulting in lesser activity in educational buildings.




==> device_analysis.tex <==
\section{Empirical Analysis of user devices}
\label{sec:device_analysis}

In today's world, most of us carry more than one mobility device. In our study, we found that each mobile device associated with a user has it's own mobility trace and displays different mobility characteristics. In this section we share the results of empirical analysis of the multiple user devices associated with a user. We divide all the mobile devices associated with a user in 3 different categories. Of all the devices associated with a user, the device that shows the most transitions in the trajectory of the device is termed as a primary device followed by secondary device and then tertiary and other devices. This division of devices results in around 93\% of the users on campus have a primary device. For the rest 7\% of the users who do not have a primary device they have a secondary device such as a laptop that doe not show transitions during mobility. Also, these users correspond to the set of users who do not have a smartphone with WiFi capabilities.

In a campus environment a typical user visits a location spends some time at that location performing some activity. Most of the users move between locations spending different amounts of times at different locations. We term the locations visited by the users as Locations of Interest [LoI]. Each location has a number of AP's associated. When a user roams around the campus from one location to another, the devices get associated with different AP's based on the type of device, aggresiveness of the device, if the device is visible on the network. 

Figure ~\ref{fig:KDE_Plots_devices} shows the density plot of time spent on campus to the number of AP's a device gets associated with over the course of the day. We see that primary devices show the highest mobility spanning to 175+ AP associations. Whereas, secondary devices and tertiary devices show substantially less mobility compared to the primary device. We also, see that the density plot of secondary and tertiary devices are very similar in nature depicting a high corelation coefficient between secondary device and tertiary devices mobility trajectory. The trajectory corelation coefficient falls in the range of 0.83-1.0 for secondary and tertiary devices where as is in the range of 0.17-0.75 for primary device trajectory and secondary device trajectory.

\begin{figure}[H]
\includegraphics[width=3.1in]{./Figures/device_timespent_apsvisited_kde_cluster.pdf}\\
\vspace{-0.2in}
\caption{KDE Plot of Time spent on campus v/s number of AP's the device gets associated with over the course of a day.}
\vspace{-0.05in}
\label{fig:KDE_Plots_devices}
\end{figure}



==> device_mobility.tex <==
\subsection{Characterizing Devices by Type}
Having analyzed the number of devices owned per user, we next analyze the {\em types}
of devices own by  users. Our wifi logs only contain the anonymized MAC address for each device, which is insufficient to determine the device type, and consequently  we must infer the device type through other means. To do so, we develop a simple method to classify devices based on their {\em mobile behavior during inactive periods}, which provides a strong indicator of the device type.  Our classification method is based on the power saving behavior of devices. Small devices
such as phones, and many tablets, tend be powered on at all times---even when the user
does not actively use the device. When these devices become idle, their network interfaces  enter a low-power listen state but stay powered up (e.g., to receive push notifications, chat messages, or video calls). Hence the device  continues to maintain a network presence (and thus is periodically visible to the wifi network).  Consequently, when a user walks from one location to another, the access points along the path periodically see the presence of the device (through scans, association or disassociation messages). Of course, if the user actively uses their device when walking, the device maintains a continuous, rather than periodic, network presence along the path. Either way, the  trajectory of the device while walking from one location to another is  visible to the network for such always-on  devices.

 
In contrast, larger mobile devices such as laptop tend to hibernate when not in active 
use (e.g., when the laptop lid is closed). The hibernate power state results in 
network interfaces being powered down, and the device no longer maintains a network
presence while hibernating. Consequently, when a user walks with a laptop
from one location to another, the device is not visible to the network during the walk
and only becomes visible when user begins using the device at the new location. 
Thus, hibernating devices exhibit
%do not exhibit a network presence during a transition from one location to another, and its mobile presence is simply 
a sequence of visible stationary periods with invisible transitions in between. Any device with aggressive OS power saving features such as laptops and e-readers exhibits this behavior. 

This difference in mobile behavior during transitions enables us to classify devices as always-on or  hibernating devices.  In our current environment, the most common always-on device is a phone, while the most common hibernating device is a laptop.\footnote{Smart watches, which are another type of always-on device, were not present in our dataset since they do not support wifi networks requiring RADIUS authentication. Tablets, which also exhibit phone-like network presence, are present on our campus but in far smaller numbers than phones.}
 Devices such as desktops, gaming consoles and wireless printers were present in our dataset, but are considered as fixed, rather than mobile devices  since they never move locations (and are filtered out from our analysis).

% with tablets being a distant second; smart watches which are growing in 
%popularity are not present in our dataset since, until recently, such devices were only able to  connect to personal wi-fi networks and not to enterprise wi-fi networks with RADIUS authentication. The most common type of hibernating device in our environment
%is a laptop. Recall that 

\begin{table}[H]
    \begin{minipage}{.4\textwidth}
      \centering
      \begin{tabular}{cc}
        \toprule Device Characteristics & \% Devices\\
	 \midrule Hibernating  & 26.91\% \\ 
	          Always-on  & 73.08\% \\
        \bottomrule
      \end{tabular}
	\caption{Distribution of always-on and hibernating devices.}
	\label{tab:tab1}
    \end{minipage}
    \hspace{0.6cm}%
    \begin{minipage}{.4\textwidth}
      \centering
      \begin{tabular}{cc}
        \toprule  Device Type & \% Users \\
	\midrule Primary  & 89.54\% \\
 		 Secondary  & 94.52\% \\
        \bottomrule
      \end{tabular}
      \caption{Ownership of primary and secondary devices.}
	\label{Tab:tab2}
    \end{minipage}
\end{table}

% \begin{table}[t]
%\begin{center}
% \begin{tabular}{||\ | c||} 
% \hline
% Secondary device type & \% Device \\ [0.5ex] 
% \hline\hline
% Hibernating  &  86.73\% \\ 
% \hline
% Always-on  & 13.27\% \\ [1ex] 
% \hline
%\end{tabular}
%\caption{Distribution of secondary devices.}
%\label{tab:tab3}
%\end{center}
%\end{table}
 
 Table \ref{tab:tab1} shows the results of our classification method across all devices
 in our dataset. As shown, 73.08\% of all devices maintain a network presence during
 location transitions and are classified as always-on devices. The remaining 26.91\% 
 devices do not exhibit any presence during location transitions and are classified as
 hibernating devices.

For the purpose of our study, we further classify all devices belonging to each user as
primary and secondary.  A  user's {\em primary} device is defined to the always-on device  that exhibits the greatest mobility (greatest number of stationary periods per day) among all always-on devices owned by that users.  All other devices belonging to that user,   whether always-on or hibernating, are defined to be secondary devices.  By virtue of being the user's most mobile device, the primary device also provides the best approximation  of the user's actual mobile behavior.
With high likelihood, a user's primary device is likely to be a mobile phone.  Further, with high likelihood, a hibernating secondary device belonging to the user is likely to a laptop.  After labeling devices as always-on and hibernating and then partitioning each user's devices as  primary and secondary, we see in Table \ref{Tab:tab2}  that 89.54\% of users own a primary device. This also implies that 10.45\% of our users do not own a smartphone (or any other always-on device).  The table shows that  94.52\% of  our users own at least one secondary device. Of these 89.54\% users who own a primary device we also find that 54.84\% of them also own a hibernating secondary device while 59.37\% own an always-on secondary device. Of all the secondary devices in our dataset,
48.02\% of them are hibernating devices, and the remaining  51.979\% are always-on secondary devices.  
%, which provides an excellent environment to study how small and large devices differ in their mobile behavior despite being owned by the same user.  

{\em Observation:} The network behavior of a mobile device in idle or sleep state is a strong indicator of the device type. Over 89\% of our campus users own a phone-like primary device, and more than 50\% of campus users own both a laptop-like hibernating device and an always-on device like phone.

\subsection{Characterizing Device Mobility}
\label{sec:device_mobility}

\begin{figure*}
\begin{minipage}[c]{0.48\linewidth}
\includegraphics[width=\linewidth]{./Figures/device_timespent_apsvisited_kde_cluster.pdf}\\
%\vspace{-0.2in}
\caption{Density plot of device active time}
%\caption{Density Plot of active time spent by devices and number of APs associated: Different mobility patterns are shown by different types of devices, with Primary device showing highest mobility. Also, Secondary and Tertiary devices have higher mobility coefficient of co-relation compared to Primary devices.}
\vspace{-0.05in}
\label{fig:device_time_density}
\end{minipage}
\hfill
\begin{minipage}[c]{0.48\linewidth}
\includegraphics[width=\linewidth]{./Figures/stationary_period_kdeplot_3n_percentage.pdf}
%\vspace{-0.2in}
\caption{Stationary Periods}
\vspace{-0.05in}
\label{fig:AP_stationary}
\end{minipage}%
\end{figure*}

\begin{figure*}
\includegraphics[width=\linewidth]{./Figures/Trajectory_timeline.pdf}\\
%\vspace{-0.2in}
\caption{Trajectory Timeline of Primary and Secondary device of a user}
\vspace{-0.05in}
\label{fig:traj_timeline}
\end{figure*}

To characterize the nomadic behavior of different types of devices, we analyze the trajectory of each device over the course of a day; the trajectory consists of a sequence of AP associations across the campus. As explained in Section \ref{sec:dataset}, AP associations of duration's that exceed the ten minute threshold represent stationary periods in the trajectory, while shorter associations are part of a transition.\footnote{When a device is at the boundary of the range of two adjacent APs, it may ping pong between the two APs even in the absence 
of any movement. We treat such scenarios as a stationary period if this behavior persist for more than the threshold duration. } Consequently, the daily trajectory of a device
comprises a sequence of alternating stationary periods and transitions to the next location. 

%A device with greater mobility will exhibit a larger number of AP associations  per day
%than one with lower mobility. 
Figure ~\ref{fig:device_time_density} shows the density 
plot of the number of AP associations for different device types and the number of hours
spent by the device on campus (defined as the time between the first time the device is visible to the network each day to the last time it is visible). The density plot shows a bimodal distribution of devices depending on whether the device belongs to an on-campus or an off-campus user;  devices belonging to off-campus users spend 8.5 hours per day,
on average, on campus, while those belonging to on-campus users (those who live on campus)
typically spend the entire day on campus.
Importantly, a user's primary device visits 75.36 APs per day, on average, for on-campus users and 37.71 APs per day, on average, for off-campus users. There is a sharp reduction in mobility for secondary devices; such devices visit 12.27 APs per day for on-campus users and 10.43 APs per day, on average, for off-campus users, which is an about 3X lower than that for primary devices.

Since primary devices are always-on devices, they maintain a network presence during user movement and consequently are seen by more APs. Not all secondary devices are always-on devices and hibernation during transitions will inherently reduce the number of APs that see the device even through the user may take the device with them where they go. To analyze whether secondary devices truly exhibit lower mobility, we must further analyze number of stationary  and transition periods, rather than raw AP associations, for each device type.  Figure \ref{fig:AP_stationary} shows the CDF of the stationary periods (i.e., AP association of ten minutes of longer) for primary and secondary devices. As shown, primary devices visit 37.84 stationary locations (i.e., have 37.84 stationary periods), on average, per day. Always-on secondary devices visit 19.54 stationary locations per day, while hibernating secondary devices visit 10.24 locations per day on average. The 90th percentile of the CDF shows that primary devices of highly mobile users visit 65 stationary locations per day, while their secondary hibernating devices visit 21 stationary locations.  The figure confirms that, even after filtering out AP associations during transitions, the number of stationary AP locations visited by primary devices is 3X higher than that of secondary devices.  Further, primary and secondary devices of highly mobile users exhibit 2X more mobility than the average user.

 The mobile behavior of primary devices deviates from 
 that of secondary devices for two reasons. First, as noted above, hibernating secondary devices do not maintain a network presence during user movement, even though the user may be carrying
 both the primary and secondary device with them. Second, users tend to take their primary 
 devices with them everywhere they go (e.g., to lunch), but they may leave larger devices 
 such as laptops behind, causing the trajectories of the primary and secondary devices
 to deviate (which also results in reduced mobility for secondary devices).  Figure \ref{fig:traj_timeline} illustrates these differences by depicting  primary and secondary device trajectory for particular user. As shown, both devices visit
 the same location whenever the users brings both devices to that location; in some cases, however,  the user leaves the laptop behind (e.g., building 4) while taking the primary device to  other buildings. In one case (building 3), the user takes the primary device to multiple  locations inside the building while leaving the laptop at one location. %Transition times representing walks from one location to another are also shown. 
To evaluate such differences across all  users,
we  computed the similarities in the trajectories of primary and secondary devices for each user using Pearson model to compute the coefficient correlation. A value of 0.5 or higher on the pearson model denotes strong correlation, while a value lower than 0.5 indicates a weak correlation. We found that the trajectory correlation coefficient between the primary and secondary device varies from 0.17-0.75 for different users, which also indicates that two types of  devices exhibit varying degrees of similarity in their daily trajectories but can also have frequent  deviations based on user behavior.

% and those of the secondary devices;  The trajectory correlation coefficient is
% only 0.17-0.75 for primary device trajectory and secondary device trajectory, while
% it is between  0.83-1.0 for secondary devices (indicating that users tend to leave behind their secondary devices in their offices or residence halls while taking their primary devices with them).
 
\iffalse
{\em Observation:} Our results show that smaller devices such as phones exhibit  atleast 3X greater mobility  than larger devices such as laptops belonging to the same  user;  devices belonging to highly mobile users, represented by the 90-th percentile of the distribution, exhibit 2X more mobility than those of the average user.  Primary and secondary device trajectories exhibit a broad range of  correlations, ranging from 0.17-0.75, indicating varying degrees of similarity in mobile behavior across a user's devices. 
\fi

   

\iffalse
**** comment out text ****
\begin{table}[t]
\begin{center}
 \begin{tabular}{||l | c||} 
 \hline
 Device Characteristics & \% Devices \\ [0.5ex] 
 \hline\hline
 Hibernating  & 42.43\% \\ 
 \hline
 Always-on  & 57.56\% \\ [1ex] 
 \hline
\end{tabular}
\caption{Distribution of always-on and hibernating devices.}
\label{tab:tab1}
\end{center}
\end{table}

\begin{table}[t]
\begin{center}
 \begin{tabular}{||c c||} 
 \hline
 Device Type & \% Users \\ [0.5ex] 
 \hline\hline
 Primary  & 93\% \\
 \hline
 Secondary  & 76.20\% \\
 \hline
\end{tabular}
\caption{Ownership of primary and secondary devices.}
\label{Tab:tab2}
\end{center}
\end{table} 

Now, that we know the distribution of devices let us analyze the mobility of these devices by answering the below questions:

\begin{itemize}
    \item How many APs do devices visit?
    \item How many locations of interest do devices visit? [Add location of interest definition in the dataset]
    \item How similar are the device trajectories of multiple devices with a single owner?
    \item What percentage of the time are the devices active?
    \item Can we derive the spatiotemporal device dynamics of all devices?
\end{itemize}

\par
The trajectory of a mobile device over the course of a day comprises of associations with multiple APs across the campus. Some associations are for longer durations representing a stationary segment when a user device stays at one place when the user performs activities like attending a class, working in the lab or staying in the dorm room. Other associations are short and in the logs, we see hops and drifts from one AP to another representing transition. These transitions represent a state of movement when the device moves from one location to another. All devices may or may not show stationary and transition segments of the trajectory. The number of APs a device gets connected to also represents its mobility, except in the case of ping-pongs, where a device keeps ping-ponging between different APs in spite of no movement. To sum, a device that has high mobility will have a higher number of associations with APs across campus than the number of AP associations by a device with low mobility.

\par
In the earlier section, we found that ~90\% of users on campus have up to 3 devices. So, we define 3 main device categories: primary device, secondary device and tertiary, and other devices. A primary device is defined as a device that shows at least one transition and has the highest mobility among the other user-owned devices, the mobility clause is used to resolve ties if any. A secondary device may or may not show transitions and shows less mobility than the primary device. The category of least mobile devices is termed as tertiary and other devices in case of ties between the mobility of secondary and tertiary devices of a user, we label the device that gets registered first on the network as secondary and the other as tertiary device. This division of devices results in around 93\% of the users on campus to have a primary device. For the rest 7\% of the users who do not have a primary device, they have a secondary device or secondary and tertiary device that does not show transitions during mobility. Also, these users correspond to the set of users who do not have a smartphone with WiFi capabilities.


Figure ~\ref{fig:device_time_density} shows the density plot of the number of APs a device gets associated with over the course of a day and number of hours the device spends on campus. The number of hours the device spends on campus is computed as the time between the first and the last presence event associated with the device in the syslog. We found that primary devices associated with 2-160 APs on a weekday, secondary devices got associated with 1-20 APs and tertiary and other devices got associated with 2-18 APs. The primary reason for such a large variation is that according to the definition primary device must show transition. When a device shows a transition in its trace it is moving between locations resulting in drifts across multiple APs on the network resulting in a large number of AP associations. Secondary and tertiary devices such as laptops mostly do not show transitions since they are in use on the network at a specific location where the device is associated with a single AP showing stationary segment. Mostly, during transitions devices such as laptops are closed and we see them associating at a new location after some time. Hence, we rarely see the phenomenon of AP drift for laptops. Also, most devices such as mobile phones are very aggressive with respect to AP hopping when compared to devices such as laptops resulting in a low number of AP associations. From figure ~\ref{fig:device_time_density} we also see that secondary and tertiary devices show a similar trend in behavior with respect to the number of APs visited as compared to that of primary devices. For users who own 3 or more devices, we found that the device trajectory of secondary and tertiary devices showed a high correlation coefficient than that with the primary device trajectory. The trajectory correlation coefficient falls in the range of 0.83-1.0 for secondary and tertiary devices whereas falls in the range of 0.17-0.75 for primary device trajectory and secondary device trajectory. Figure ~\ref{fig:device_LoI} shows that primary devices visit an average of 5.64 locations of interest per day, whereas secondary and tertiary devices visit 3 locations per day. Thus, we can conclude that all the mobile devices do not have similar mobility characteristics. If a user owns multiple devices, each device can show a different set of mobility attributes.

\par
Next, we try and analyze the trajectory timelines of the devices to find the spatiotemporal mobility dynamics. Since each user has a different mobility pattern we definitely see a different device mobility patterns between users. However, we analyze the device mobility pattern within a user device set to understand the differences in spatiotemporal device mobility and their underlying reasons. For this, we take a few sample trajectories of devices owned by a single user and plot the trajectory. We find that there are 2 main scenarios which result in different mobilities for devices owned by a single user. Scenario 1 is illustrated in figure ~\ref{fig:}, here the user moves around with only the primary device while the secondary device stays at a particular location. Such a scenario may arise when a user goes out to pick a quick cup of coffee or to grab food. In such cases, while the primary device shows associations with APs across other buildings the secondary device doesn't show any change in its associations resulting in lesser mobility.

Scenario 2 is illustrated in figure ~\ref{fig:}, here a secondary device appears at a location and then, disappears from the network for some time, reappearing at a new location. Whereas, the primary device shows a complete trajectory comprising of the transitions also. In such cases, we can safely assume that the primary device is a mobile phone that is turned on and visible on the network always and gets carried by the user around. Whereas the secondary device is a device such as a laptop that gets associated when is turned on and used by the user but during the users transitions between locations the laptop gets closed and goes off to sleep mode getting disconnected from the network. Once, the user reaches the destination and re-opens the laptop, it gets associated with the AP at the new location, this is shown in the WiFi logs by disappearance and appearance of the devices on the campus.

*** comment out ***
\fi


==> related.tex <==
\section{Related Work}
\label{sec:related}
Human movements have been studied in great detail for urban planning and for inferring the dynamics of cities. The work done on human mobility can be divided into 3 main categories. Firstly, work done on identification of patterns of movement. The work on understanding human mobility pattern ~\cite{gonzalez08, Zheng:2008:UMB:1409635.1409677, Ganti:2013:IHM:2493432.2493466} indicates that the spatio-temporal patterns of human movements show a high degree of regularity and repeatability. Secondly, research on identification of the behavioural factors that cause the human movement or the reason for change in location, ~\cite{jiang2012clustering, Axhausen2002, Jiang2012, 725, Lane:2014:CPS:2632048.2636094}. Determination of the means of transportation, direction of movements, activity associated with the movement, distance travelled, important places of visit or Points of Interest (POI), commuting patterns and clusters of people. Thirdly, work associated with prediction of next location and modeling mobility of people ~\cite{Ganti:2013:IHM:2493432.2493466, Lee:2006:MST:1132905.1132915, Do:2012:CCM:2370216.2370242, kim2006extracting, DBLP:journals/corr/PappalardoS16, Lin:2012:PIM:2370216.2370274}. The spatio-temporal data used for these studies came from various sources such as GPS, CDR/GSM, WiFi, surveys and taxi logs.

While knowledge of time and location of people clustering for activities, location of important places for gatherings or tourist travel is important from economic and social perspective, there is no work done on the mobility of the multiple devices owned by a user and the co-relation of the trajectories of those devices. Also, while studies mainly concentrate on place of work and type of activities, our work takes into consideration the fact that in a commerical place such as a college campus, technology park or a city each building has a different purpose or activity assigned to it and so, the mobility of users inside a building is different from that of mobility between buildings. In this work we find that not only does each individual user have a regularity in mobility driven by his or her own schedule but there is a collective regularity among all the users across the campus inspite of users having their own distinct schedule. 

%A commerical space such as a campus environment that has different kinds of structural buildings each serving a different purpose emulates the environment of a city, a technology park or an industrial complex. If, we define nomadicity to cover the stay periods and in-transit periods of a user with regard to accomplishing the assigned work based on the availability of resources at different sites within the campus; we find that each user has a repeatability in nomadicity pattern based on the users schedule of classes or work schedule depending on the role of the user on campus. Further, we use data mining concepts to find the structure in the nomadicity pattern of the entire population of users. We apply clustering to find rhythms followed by users. Additionally, we find the hidden framework in daily nomadicity patterns of users and cluster them into various groups. We also, use data mining techniques to identify collective behaviour of users on campus and also to distinguish spectators from participants in a crowd activity. The empirical analysis done in this paper helped us to further design a model for nomadicity of users on campus. This model is extremely useful to understand the nomadicity and dynamics of campus, commercial space or a city.



==> results.tex <==
\section{Experimental Results}
\label{sec:results}
%In this section, we present a subset of the most interesting observations and findings of our work. In each of the following sub-sections, we construct series of questions related to devices, users, mobility and answer them based on the data.

In this section, we present empirical results for campus-scale mobility obtained from our analysis of the campus wifi dataset. 

\input{devices_users}
\input{device_mobility}
%\input{bldg_analysis}
\input{inter_bldg_analysis}
\input{intra_bldg_analysis}


==> secondarydevice.tex <==
\subsection{Secondary Device Distribution}
\label{sec:secondarydevice}

\begin{figure*}
\begin{tabular}{cc}
\includegraphics[width=3in]{./Device_distribution/fac_bldghistogram_by_day.pdf}&
\includegraphics[width=3in]{./Device_distribution/sec_fac_bldghistogram_by_day.pdf} \\
(a) Primary device & (b) Secondary device
\end{tabular}
\vspace{-0.2in}
\caption{Buildings visited by primary and secondary device of faculty staff by day of the week}
\vspace{-0.05in}
\label{fig:fac_bldgs}
\end{figure*}


\begin{figure*}
\begin{tabular}{cc}
\includegraphics[width=2.1in]{./Device_distribution/stud_bldghistogram_by_day.pdf}&
\includegraphics[width=2.1in]{./Device_distribution/sec_stud_on_bldghistogram_by_day.pdf} \\
(a) Primary device & (b) Secondary device
\end{tabular}
\vspace{-0.2in}
\caption{Buildings visited by primary and secondary device of students by day of the week}
\vspace{-0.05in}
\label{fig:stud_bldgs}
\end{figure*}

\begin{figure*}
\begin{tabular}{cc}
\includegraphics[width=2.1in]{./Device_distribution/fac_entryexit_non_stationary.pdf}&
\includegraphics[width=2.1in]{./Device_distribution/stud_off_entryexit_all.pdf} \\
(a) Entry Exit time KDE plot for faculty staff & (b) Entry Exit time KDE plot for off-campus students
\end{tabular}
\vspace{-0.2in}
\caption{Entry Exit time KDE plot by role of secondary devices}
\vspace{-0.05in}
\label{fig:eekde}
\end{figure*}

In this section, we compare the device nomadicity. Based on the authorization messages in the syslog we found a mapping between the devices and users. On analyzing the nomadicity of devices associated with a user we found that not all devices associated with a user showed the same nomadicity trajectories. Different devices showed different levels of nomadicity, due to difference in usage. We found that some user devices were stationary and showed no changes in location whereas others showed changes in locations over the course of the day. When a user is mapped to multiple devices, we term the device that shows the most nomadicity as primary device while, the next most nomadic device is termed as secondary device. For the analysis of distance walked, frequent paths, modeling and all other sections of the paper we use the primary device. In this section, we present our analysis of the nomadicity of secondary devices. Also, we found that it is easy to differentiate between stationary and non-stationary devices. We filter out the devices that are associated with the same Access Point for the entire working time duration or for 24 hours of a day as a stationary device. Also, few devices have multiple users logging into it. Such, devices were not associated with any one user and most of such devices were found to be stationary devices.

Figure ~\ref{fig:fac_bldgs} shows the histogram of the buildings visited by devices identified as primary and secondary over the course of the entire semester. We observe that the number of buildings visited by primary devices has a higher span than the number of buildings visited by secondary device, also, the count of primary devices that visits the buildings on campus over the entire semester is higher than that of secondary devices, showing that not all devices associated or carried by an individual has the same nomadicity. We make a similar observation for student devices as shown in ~\ref{fig:stud_bldgs}.

However, for exit entry time for different roles for different days of the week, as shown in Figure ~\ref{fig:faceetime}, Figure ~\ref{fig:studeetime} and Figure ~\ref{fig:eekde} we make similar observations as that of primary devices.

